Bonsai: Interpretable Tree-Adaptive Grounded Reasoning

To develop general-purpose collaborative agents, humans need reliable AI systems that can (1) adapt to new domains and (2) transparently reason with uncertainty to allow for verification and correction. Black-box models demonstrate powerful data processing abilities but do not satisfy these criteria due to their opaqueness, domain specificity, and lack of uncertainty awareness. We introduce Bonsai, a compositional and probabilistic reasoning system that generates adaptable inference trees by retrieving relevant grounding evidence and using it to compute likelihoods of sub-claims derived from broader natural language inferences. Bonsai's reasoning power is tunable at test-time via evidence scaling and it demonstrates reliable handling of varied domains including transcripts, photographs, videos, audio, and databases. Question-answering and human alignment experiments demonstrate that Bonsai matches the performance of domain-specific black-box methods while generating interpretable, grounded, and uncertainty-aware reasoning traces.

==> content/08_ethics.tex <==
\section{Limitations}
While the probability scoring system outperforms other prompting techniques and some uncertainty calibration approaches, there is little evidence that the intermediate probability scores reflect only the evidence that has been explicitly acknowledged thus far. For the sake of transparency, it would be helpful for future work to analyze the relationship between intermediate scores and final scores, and to develop a truly iterative approach in which the model is not provided with all evidence at once.

==> prompts/h_gen_tvqa.tex <==
\prompt{Hypothesis Generation (Multiple Choice - TVQA, ARC)}{
Convert each of the answer options for the following questions into GRAMMATICAL
ANSWER SENTENCES. Make sure that they are FULL and COMPLETE sentences, not just
words. They should be sentences that you can "prove" by reasoning about the
situation. Proving the sentence should amount to choosing choosing that answer
option over the other one(s).\\

QUESTION: What was in the back of Zoey's van after she opened the doors?\\

ANSWERS:\\
(1) A dog with a broken leg.\\
(2) Stolen electronics.\\
(3) Bunnies.\\
(4) A romantic dinner.\\
(5) A desk to put together.\\

SENTENCES:\\
(1) A dog with a broken leg was in the back of Zoey's van after she opened the doors.\\
(2) Stolen electronics was in the back of Zoey's van after she opened the doors.\\
(3) Bunnies were in the back of Zoey's van after she opened the doors.\\
(4) A romantic dinner was in the back of Zoey's van after she opened the doors.\\
(5) A desk to put together was in the back of Zoey's van after she opened the doors.\\

\{questions\}\\

SENTENCES:
}

==> prompts/probability_cf.tex <==
\prompt{Counterfactual prompt addition}{
As additional information, you know that one of the five following statements is true about this situation:\\
\{answers\}\\

Given this, determine the likelihood that the following hypothesis is true.
}

==> prompts/summarize.tex <==
\prompt{Summarization (Transcript)}{Write a very brief summary describing the genre of the following transcript. An example summary is "Some people discuss a political development." Your summary should not be more than seven words. Respond with your summary, and nothing else.\\

TRANSCRIPT:\\
\{dialogue\}\\

SUMMARY:}
